On the Benefits of Memory for Modeling Time-Dependent PDEs

Data-driven techniques have emerged as a promising alternative to traditional numerical methods for solving PDEs. For time-dependent PDEs, many approaches are Markovian -- the evolution of the trained system only depends on the current state, and not the past states. In this work, we investigate the benefits of using memory for modeling time-dependent PDEs: that is, when past states are explicitly used to predict the future. Motivated by the Mori-Zwanzig theory of model reduction, we theoretically exhibit examples of simple (even linear) PDEs, in which a solution that uses memory is arbitrarily better than a Markovian solution. Additionally, we introduce Memory Neural Operator (MemNO), a neural operator architecture that combines recent state space models (specifically, S4) and Fourier Neural Operators (FNOs) to effectively model memory. We empirically demonstrate that when the PDEs are supplied in low resolution or contain observation noise at train and test time, MemNO significantly outperforms the baselines without memory -- with up to 6x reduction in test error. Furthermore, we show that this benefit is particularly pronounced when the PDE solutions have significant high-frequency Fourier modes (e.g., low-viscosity fluid dynamics) and we construct a challenging benchmark dataset consisting of such PDEs.

==> ICLR_2025_Template/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Sections/Mori-Zwanzig.tex <==
\section{Mori-Zwanzig Theory}
The Mori-Zwanzig formalism (\cite{Zwanzig2001}) uses dependence on the past states of a system to compensates for the loss of information that arises when such system is only partially observed. In our PDE setting, partial observation can mean several things: observing the solution at a discretized grid in space, only observing the Fourier modes up to a critic frequency, or having noisy observations of the solution.

In particular, the Mori-Zwanzig formalism applied to time-dependent PDEs is well-known in the Physics literature and known as the Nakajima–Zwanzig equation (\cite{nakajima-transport}). We will briefly expose this equation applied to our setting.

For a given spatial dimension $d$, let $\Omega$ be an open set in $\mathbb{R}^{d}$ and $L^2(\mathcal{D};\mathbb{R})$ the set of square integrable functions from $\mathcal{D}$ to $\mathbb{R}$. Our PDE can be written as: 
\begin{align}
    \label{eq_MZ:PDE}
    \frac{\partial u}{\partial t} (t,x) &= \mathcal{L}[u] (t,x) \quad (t,x)\in[0,T]\times\mathcal{D} \\
    u(0,x) & = u_0(x) \quad x \in \mathcal{D}
\end{align}

plus some boundary conditions. Now let $\mathcal{P}: L^2(\mathcal{D};\mathbb{R}) \rightarrow L^2(\mathcal{D};\mathbb{R}) $ be a linear projection operator that satisfies $\mathcal{P}^2=\mathcal{P}$. Let $\mathcal{Q}=I - \mathcal{P}$, where $I$ is the identity operator. In our setting, for the PDE solution at timestep $t$ $u_t \in L^2(\mathcal{D};\mathbb{R})$, $\mathcal{P}[u_t]$ is the part of the solution that we observe and $\mathcal{Q}[u_t]$ is the unobserved part. In our problem, the initial information we receive for the system is $\mathcal{P}[u_0]$. Then, applying $\mathcal{P}$ and $\mathcal{Q}$ to \ref{eq_MZ:PDE} and using $u = \mathcal{P}[u] + \mathcal{Q}[u]$, we get:
\begin{align}
    \label{eq_MZ:PDE_P}
    \frac{\partial }{\partial t} \mathcal{P}[u] (t,x) &= \mathcal{P} \mathcal{L}[u] (t,x) = \mathcal{P} \mathcal{L} \mathcal{P} [u] (t,x) + \mathcal{P} \mathcal{L} \mathcal{Q} [u] (t,x)  \\
    \label{eq_MZ:PDE_Q}
     \frac{\partial }{\partial t} \mathcal{Q}[u] (t,x) &= \mathcal{Q} \mathcal{L}[u] (t,x) = \mathcal{Q} \mathcal{L} \mathcal{P} [u] (t,x) + \mathcal{Q} \mathcal{L} \mathcal{Q} [u]  (t,x)
\end{align}
Solving for \ref{eq_MZ:PDE_Q} yields: 
\begin{align*}
    \mathcal{Q}[u](t,x) = e^{\mathcal{Q} \mathcal{L} t} \mathcal{Q}[u_0](t,x) + \int_0^t \exp{\mathcal{Q}\mathcal{L}(t-s)} \mathcal{Q}\mathcal{L} \mathcal{P}[u](s,x) ds
\end{align*}

Plugging into \ref{eq_MZ:PDE_P}, we obtain a Generalized Langevin Equation \citep{mori1965transport} for $\mathcal{P}[u]$:

\begin{align}
    \label{eq_MZ:GLE}
    \frac{\partial }{\partial t} \mathcal{P}[u] (t,x) & = \mathcal{P} \mathcal{L} \mathcal{P} [u] (t,x) + \mathcal{P}\mathcal{L} \int_0^t \exp{\mathcal{Q}\mathcal{L}(t-s)} \mathcal{Q}\mathcal{L} \mathcal{P}[u](s,x) ds + \mathcal{P} \mathcal{L} e^{\mathcal{Q} \mathcal{L} t} \mathcal{Q}[u_0](t,x)
\end{align}

We will refer to the first summand on the right hand side of \ref{eq_MZ:GLE} as the \textit{markovian} term because it only depends on $\mathcal{P}[u](t,x)$, the second summand as the \textit{memory} term because it depends on $\mathcal{P}[u](s,x)$ for $0\leq s \leq t$, and the third summand as the \textit{initial unobserved residual} as it depends on $\mathcal{Q}[u_0]$ which is never observed.

Nevertheless, solving $\ref{eq_MZ:GLE}$ is almost as difficult as solving the full system \citep{moriks-Ma2018-up, nakajima_derivation-Breuer2002}. In the Physics literature, the memory term has been approximated through a perturbation expansion of the exponential \citep{nakajima_derivation-Breuer2002}, or by approximating the operator $\exp{\mathcal{Q}\mathcal{L}(t-s)}:L^2(\mathcal{D};\mathbb{R}) \rightarrow L^2(\mathcal{D};\mathbb{R})$ through operators defined in  $\mathcal{P}[L^2(\mathcal{D};\mathbb{R})]$ \citep{shigeva1-shi2003new,shigeva2-zhang2006nonequilibrium,shigeva3-10.1063/1.4948408,shigeva4-10.1063/1.4948612}. In a Machine Learning context, \citet{moriks-Ma2018-up} develop a hybrid approach where the memory term was approximated with an LSTM \citep{LSTM-10.1162/neco.1997.9.8.1735}, and then used as input of a numerical solver. In this work, we treat the whole memory term as an operator $\mathcal{M}: \mathcal{C}\left([0,T],\mathcal{P}[L^2(\Omega;\mathbb{R})]\right) \rightarrow \mathcal{P}[L^2(\Omega;\mathbb{R})]$ to be approximated by a parametrized layer of a neural network, which is the motivation for our architecture.

==> Sections/challenges_high_frequency.tex <==
% \section{Challenges of high frequency solutions}
% Most results of state of the art Neural Operators are given for datasets in which Fourier modes above the Nyquist frequency are negligible. For a given continuous function $u(x)$ with Fourier Spectrum $(\uh_k)_{k\in\mathbb{Z}}$ and a spatial resolution $f$, we can define the following quantity to assess the importance of high frequency modes in the solution:
% \begin{equation}
%     \omega = \frac{\sum_{|k|\geq\frac{f}{2}} \|\hat{u}_k\|}{\sum_{k\in\mathbb{Z}} \|\hat{u}_k\|}
% \end{equation}

% Naturally, $0\leq \omega \leq 1$. When $\omega$ is close to zero, the signal is mostly composed of low frequencies, whereas when $\omega$ is closer to 1, the high frequencies components are significant.

==> Sections/method_DFT.tex <==
\section{Method}
\subsection{Setup}
Throughout the rest of this section, we will denote $d\in\mathbb{N}$ the spatial dimension of our PDE, $\mathcal{D}$ and open and bounded subset of $\mathbb{R}^d$,  and $[0,T]\subset \mathbb{R}$ an interval in $\mathbb{R}$.

\begin{nota}
    ($L^2(\mathcal{D})$). We will denote by $L^2(\mathcal{D})$ the Hilbert Space of integrable complex-valued periodic functions equipped with the inner product:
    \begin{align*}
        \langle u, v \rangle = \int_\mathcal{D} u(x) \overline{v(x)} dx
    \end{align*}
\end{nota}
\begin{nota}
    ($l^2(\mathbb{Z}^d$)). We will denote by $l^2(\mathbb{Z}^d$) the Hilbert Space of summable complex-valued sequences equipped with the inner product: 
    \begin{align*}
        \langle a, b \rangle = \sum_{k\in \mathbb{Z}^d} a_k \overline{b_k}
    \end{align*}
\end{nota}
\begin{lemma}
    (Parseval Identity) $L^2(\mathcal{D})$ and $l^2(\mathbb{Z}^d)$ are isometrically isomorphic.
\end{lemma}
\begin{defi} (First order temporal PDE with boundary conditions)
    A first order temporal PDE with periodic boundary conditions is a PDE that can be expressed as: 
    \begin{align}
    \label{PDE}
    \frac{\partial}{\partial t} u (t,x) & = \mathcal{A}[u] (t,x) \quad (t,x) \in [0,T] \times \mathcal{D} \\
    u(0,x) &= g(x) \\
    u(t,x)|_{\partial \mathcal{D}} &= K
    \end{align}
    Where $\mathcal{A}$ is a differential operator in $x$, $g \in L^2(\mathcal{D})$ and $K\in\mathbb{R}$.
\end{defi}

\begin{defi} (Space-time equivariant linear differential operator)
A space-time equivariant differential linear differential operator is a linear differential operator that can we written as: 
\begin{align*}
    \mathcal{A} = \sum_{\alpha \in \mathcal{A}} a_{i} \frac{\partial^{|\alpha|}}{\partial^{\alpha_1}x_1 ... \partial^{\alpha_d}x_d}
\end{align*}
where $\mathbb{A} \subset \mathbb{N}^d$ 
is a finite set and $a_i \in \mathbb{C}$ are the coefficients of the PDE
that are independent of both space and time.
\end{defi}
\tm{use $|\alpha|$ as the index for $a$ instead of $i$. Also mention 
the multiset notation everywhere.}

\begin{definition}[Continuous Fourier Transform]
    
\end{definition}

\begin{defi} (Space-time equivariant first order temporal PDE with boundary conditions)
A space-time equivariant first order temporal PDE is a first order temporal PDE with boundary conditions where the operator $\mathcal{A}$ is space-time equivariant. 
\end{defi}

\begin{defi} (Continuous time Fourier Transform (1D))
    For a periodic function $u\in L^2(\mathcal{D})$, we define its continuous time Fourier Transform by $\uh=(\uh_k)_{k\in\mathbb{Z}^d}$ where: 
    $$u_k = \int_{\mathcal{D}}u(x) \exp{-i 2\pi \langle x , k \rangle}dx$$
\end{defi}

\begin{defi} (Equispaced grid with $f$ points). Let  $K\in\mathbb{R}$ with  $K>0$. An equispaced grid with $f$ points in $[0,L]$ is a sequence of $f$ points $(x_n)_{n=0}^{f-1}$ given by $x_n = n \frac{K}{f}$.
\end{defi}
\begin{defi} (Discrete Fourier transform (1D))
    For $d=1$, $u\in L^2([0,L])$ and an equispaced grid in $[0,L]$ with $f$ points, we define the discrete Fourier transform of $u$ by $\ub=(\ub_k)_{|k| \leq \floor{\frac{f}{2}}}$ as: 
    $$
    \ub_k = \sum_{n=0}^{f-1} u(x_n) \exp{-i 2\pi n \frac{k}{f}}$$ 
    We will also denote $f_c=\floor{\frac{f}{2}}$.
    % For ease of notation, we will define $\ub_k(t)$ for all $k \in \mathbb{Z}$ by setting $\ub_k(t)=0$ for $|k| > f_c$.
\end{defi}


\begin{defi} (Discrete-time Fourier transform (1D))
    For $d=1$, $u\in L^2(\mathbb{R})$ and $T\in\mathbb{R}$, we define the Discrete-time Fourier transform as: 
    $$
    \hat{u}^{\frac{1}{T}}(k) = \sum_{n=-\infty}^{\infty} T u(nT) e^{-i2\pi k T n}$$
\end{defi}


\begin{lemma}
     For $d=1$, $u\in L^2([0,L])$ and an equispaced grid in $[0,L]$ with $f$ points, the Discrete Fourier Transform equals the Discrete-time Fourier transform for $T=\frac{1}{f}$: 
     $$
     \ub_k = \hat{u}^{\frac{1}{T}}(k) \quad |k|\leq f_c
     $$
\end{lemma}

\tm{isn't it true for all the points and not just the Nyquist frequency?}


\begin{lemma} (Poisson Summation Formula, 1D)
\label{lemma:poisson_summation}
    For $d=1$, $u\in L^1(\mathcal{D})$ periodic and an equispaced grid in $\mathcal{D}$ with $f$ points, the following equality holds: 
    \begin{align}
        \label{eq:possion_summation}
        \ub_k = f \sumk \uh_{k'}
    \end{align}
    % Where $T=\frac{1}{f}$.
\end{lemma}

\begin{lemma} (PDE reformulation in frequency space)
\label{PDE_reformulation}
     Given a space-time equivariant first order temporal PDE with periodic boundary conditions, there exist constants $(C_k)_{k\in \mathbb{Z}^d}$, $C_k \in \mathbb{C}$, such that the Fourier Transform of the solution $u$ satisfies: 
     \begin{align}
        \label{eq:PDE_reformulation}
         \frac{d}{d t} \uh_k (t)& = C_k \uh_k \quad k \in \mathbb{Z}^d \\
         \uh_k(0)& = \hat{g}_k
     \end{align}

\tm{write what the $C_K$ is here as part of the lemma}

\end{lemma}
\begin{proof}
Taking the continuous Fourier transform of the solution on both sides of \ref{PDE} and using the properties of the Fourier transform, we have: 
\begin{align*}
    \frac{\partial}{\partial t} \uh(t,k) &= \mathcal{F}  \circ \left(\sum_{\alpha \in \mathbb{A}} a_{i} \frac{\partial^{|\alpha|}}{\partial^{\alpha_1}x_1 ... \partial^{\alpha_d}x_d}\right)[u] (t,k) \\
    & = \left(\sum_{\alpha \in \mathbb{A}} a_{i} \prod_{n=1}^d (i k_n)^ {\alpha_n} \right) \hat{u}(t,k)
\end{align*}
    \tm{add the multiset definition and clean this up for $k$ as well.}

Our result follows from setting: 
\begin{align*}
    C_k = \left(\sum_{\alpha \in \mathbb{A}} a_{i} \prod_{n=1}^d (i k_n)^ {\alpha_n} \right)
\end{align*}
\end{proof}

\begin{ex} (1D Diffusion)
    In the case of 1D Diffusion: 
    $$ \frac{\partial}{\partial t} u(t,x) = D \frac{\partial^2}{\partial x^2} u(t,x)$$
    Then $C_k$ is given by: 
    $$
    C_k = - D k^2
    $$
\end{ex}

\tm{give example of what this 
$C_k$ looks like for advection or diffusion}

% \begin{defi}
%     A complex valued sequence indexed in $\mathbb{Z}^2$ is a sequence of complex numbers $\left(A_{kk'}\right)_{k,k'\in\mathbb{Z}}$, $A_{kk'} \in \mathbb{C}$.
% \end{defi}

% \begin{defi}
%     Given a complex valued sequences indexed in
% \end{defi}

\begin{defi} (Linear GLE)
Given $f_c, F \in \mathbb{N}$, $\beta_0 \in \mathbb{C}^{2F}$, $A^{11}\in \mathbb{C}^{(2f_c+1) \times (2f_c+1)}$, $A^{12}\in\mathbb{C}^{(2f_c+1) \times (2F+1)}$, $A^{21}\in\mathbb{C}^{(2F+1) \times (2f_c+1)}$ and $A^{22} \in \mathbb{C}^{(2F+1) \times (2F+1)}$, $T\in \mathbb{R}$. we will say that $v: [0,T]\rightarrow \mathbb{C}^{f_c}$ satisfies the Generalized Langevin Equation for $f_c$, $F$, $\beta_0$, $A^{11}$, $A^{12}$, $A^{21}$ and $A^{22}$ if: 
    \begin{equation}
        \label{eq:main_GLE}
        \frac{d}{d t} \ub(t) = A^{(11)}\ub(t) + A^{(12)}\int_0^t e^{A^{(22)} (t-s)} A^{(21)}\ub(s) ds + A^{(12)} e^{ A^{(22)} t}  \beta_0 \quad \forall t\in[0,T]
    \end{equation}

We will refer to the first summand of the right hand side as the Markov term, the second summand as the memory term, and the third summand as the initial unobserved residual.


\end{defi}


\begin{nota} (Matrix indexing)
    For convenience, instead of indexing the matrices of the Linear GLE from $0$ to $2f_c+1$ or from $0$ to $2F+1$, we will index them from $-f_c$ to $f_c$ and $-F$ to $F$. Thus, we will have $(A^{11}_{kk'})_{|k| \leq f_c, |k'| \leq F}$, $(A^{12}_{kk'})_{|k| \leq f_c, |k'| \leq F}$, $(A^{21}_{kk'})_{|k| \leq F, |k'| \leq f_c}$, $(A^{22}_{kk'})_{|k| \leq F, |k'| \leq f_c}$,
\end{nota}


\begin{obs}
    Lemma \ref{PDE_reformulation} states that in the case of Space-time equivariant first order temporal PDEs with boundary conditions, the time evolution of frequencies of the solution only depends on their initial condition, so there is no frequency fixing. However, when dealing with the discrete Fourier transform, all frequencies above the Nyquist critical frequency will contribute to the discrete Fourier transform frequencies, yielding a complex system where frequencies interact with each other. Our Main Proposition offers an equation to model this frequency mixing.
\end{obs}

\subsection{Main Proposition} 
\begin{prop}
    \label{main_prop}
    Let $d=1$. Consider a space-time equivariant first order temporal PDE and a equispaced grid in $\mathcal{D}$ with $f$ points. Let $f_c=\floor{\frac{f}{2}}$, let $C_k$ refer to the constants of the PDE reformulation in lemma \ref{PDE_reformulation} and let $\ub$ be the discrete Fourier Transform of the solution of the PDE $u$. Furthermore, suppose that $\hat{g}_k=0 \ \forall |k|\geq F$. Then, the following two properties are satisfied: 
    \begin{enumerate}[(i)]
        \item 
     $\ub$ satisfies the following Linear GLE for $f_c$, $F$, $\beta_0$, $A^{(11)}$, $A^{(12)}$, $A^{(21)}$ and $A^{(22)}$ given by:
    % \begin{align*}
    %     \beta_0 & = \uh(0) - \gamma_0 \ub(0) \\
    %     \gamma_0 & = \frac{\langle\uh(0), \ub(0) \rangle}{\parallel \ub(0)\parallel^2} \\
    %     A^{(11)}_{kk'} &= f \gamma_0 C_{k'} \delta_{kk'} & |k|\leq f_c, |k'| \leq f_c \\
    %     A^{(12)}_{kk'} & = f C_{k'} \delta_{[k][k']} & |k| \leq f_c, k' \in \mathbb{Z} \\
    %     A^{(21)}_{kk'} & =  C_{k'} \gamma_0 \left[ 1 - \gamma_0 f \right]\delta_{kk'} & k \in \mathbb{Z}, |k'| \leq f_c  \\
    %     A^{(22)}_{kk'} & = \left[\delta_{kk'}C_{k'} - \gamma_0 f C_{k'}\right] \delta_{[k][k']} & k \in \mathbb{Z}, k' \in \mathbb{Z}
    % \end{align*}
        \begin{align*}
        \beta_0 & = \uh(0) - \gamma_0 \ub(0) \\
        \gamma_0 & = \frac{\langle\uh(0), \ub(0) \rangle}{\parallel \ub(0)\parallel^2} \\
        A^{(11)}_{kk'} &= f \gamma_0 C_{k'} \delta_{kk'}\\
        A^{(12)}_{kk'} & = f C_{k'} \delta_{[k][k']} \\
        A^{(21)}_{kk'} & =  C_{k'} \gamma_0 \left[ 1 - \gamma_0 f \right]\delta_{kk'}  \\
        A^{(22)}_{kk'} & = \left[\delta_{kk'}C_{k'} - \gamma_0 f C_{k'}\right] \delta_{[k][k']}
    \end{align*}
    Where $[k]$ refers to the congruence class of $k$ modulo $f$.
    \item
    % For any other Generalized Langevin equation that can be expressed as:
    %     \begin{equation*}
    %     \frac{d}{d t} \ub(t) = \Tilde{A}^{(11)}\ub(t) + \Tilde{A}^{(12)}\int_0^t e^{\Tilde{A}^{(22)} (t-s)} \Tilde{A}^{(21)}\ub(s) ds + \Tilde{A}^{(12)} e^{ \Tilde{A}^{(22)} t}  \Tilde{\beta}_0
    % \end{equation*}
    % with $\Tilde{\beta}_0=\uh - \Tilde{\gamma}_0\ub$ and $\Tilde{\gamma}_0\in \mathbb{C}$, then:
    % \begin{equation*}
    %     ||\Tilde{\beta}_0|| \geq ||\beta_0||
    % \end{equation*}
    If $\ub$ satisfies any other Linear GLE with for $f_c$, $F$, $\Tilde{\beta_0}$, $\Tilde{A^{11}}$, $\Tilde{A}^{12}$, $\Tilde{A}^{21}$, $\Tilde{A}^{22}$ with  $\Tilde{\beta}_0=\uh - \Tilde{\gamma}_0\ub$ for $\Tilde{\gamma}_0 \in \mathbb{C}$, then: 
        \begin{equation*}
        ||\Tilde{\beta}_0|| \geq ||\beta_0||
    \end{equation*}
    
    \end{enumerate}
\end{prop}

\textit{(Proof)}
We will first prove the first part of the proposition. We can use the Poisson Formula \ref{eq:possion_summation} and the PDE reformulation formula \ref{eq:PDE_reformulation} to write:

\begin{align}
    \label{eq:prop1.1}
    \frac{d}{dt} \ub_k (t) = f \sumk C_{k'} \uh_{k'}(t) \quad |k| < f_c
\end{align}


Using the definition of $\gamma_0$ from the proposition statement, let us define the following variable:
\begin{align*} 
    \beta_k(t) := \uh_k (t) - \gamma_0 \ub_k(t)
\end{align*}

Substituting into equation \ref{eq:prop1.1} we get: 
\begin{align*}
    \frac{d}{dt} \ub_k (t) = f \gamma_0 C_k \ub_k (t) + f \sumk C_{k'} \beta_{k'}(t) \quad |k| < f_c
\end{align*}

We can also take the derivative in our definition of $\beta_k(t)$ to get: 
\begin{align*}
\frac{d}{dt} \beta_k(t) &= C_k \uh_k(t) - \gamma_0 \frac{d}{dt}\ub_k(t) \\
& = \gamma_0 C_k \left[ 1 - \gamma_0 f \right] \ub_k(t) + \sumk \left[\delta_{kk'}C_{k'} - \gamma_0 f C_{k'}\right]\beta_{k'}(t)
\end{align*}
\tm{$\beta_{k'}$ is undefined for $|k| \leq f_c$. This has to be in terms of $\hat{u}_{k'}$.}

Using the matrices definitions from the lemma statement, we have the following linear system of ODEs: 
\begin{align*}
    \frac{d}{dt} \ub (t) = A^{(11)} \ub(t) + A^{(12)} \beta(t) \\
    \frac{d}{dt} \beta (t) = A^{(21)} \ub(t) + A^{(22)} \beta(t)
\end{align*}

Solving this system of ODEs for $\beta(t)$ and substituting in the equation for $\ub(t)$ yields the Generalized Langevin Equation of the Proposition.

\begin{defi} ($\eta(t)$)
    We define the following quantity: 
    $$
    \eta(t) = 1 - f \frac{\langle\uh(t), \ub(t) \rangle}{||\ub(t)||^2}
    $$
    Note  $\eta(0) = 1 - f \gamma_0 $
\end{defi}

\begin{remark}
    The memory term in the Linear GLE of $\ref{main_prop}$ is proportional to $\eta(0) ( 1 - \eta(0) )$. Then, if $ \eta(0) ( 1 - \eta(0) ) $ is not near zero, we can expect that a Deep Learning architecture that has the choice of incorporating memory will outperform a memoryless one.
\end{remark}



\newpage



% Let $\mathcal{D}$ be an open set in $\mathbf{R}^d$,





==> Sections/notation.tex <==
\section{Background}


==> Sections/scratch.tex <==

Let $L^2([0,1] \times [0, 2 \pi])$ be the space of square integral functions. Suppose we have the following PDE with periodic boundary conditions: 


Where $\mathcal{A}$ is a differential operator on $x$. For the following theoretical analysis, we will further assume that the differential operator can be written as  $\mathcal{A}= \sum_{n=0}^N a_n \frac{d^n}{dx^n}$, $a_n \in \mathbb{R}$. That is to say, its coefficients do not depend on $x$ nor $t$. Under smoothness conditions on $\mathcal{A}$, this is equivalent to assuming that  $\mathcal{A}$ is translation equivariant in time and space: 
\begin{align*}
\mathcal{A}[u(t, x-c)] &= \mathcal{A}[u](t,x-c) \quad \forall c \in \mathbb{R} \\
\mathcal{A}[u(t-c, c)] &=  \mathcal{A}[u](t-c,x) \quad \forall c \in \mathbb{R}
\end{align*}

which is a common assumption in most physical PDEs.

We know that $\{\exp(-i k x) | k \in \mathbb{N}\}$ is a basis of the $L^2([0,1] \times [0, 2 \pi])$ periodic functions. Thus, we can apply a Fourier transform to our PDE, and because the coefficients on $\mathcal{A}$ do not depend on $x$, we will get a diagonal linear system of ODEs: 
\begin{align}
\label{lemma:uhat_t}
    \partial_t \hat{u}_k(t) & = C_k \hat{u}_k (t)  \quad t \in [0,1]  \\
    \hat{u}_k(0) &= \hat{g}_k
\end{align}

Where $k\in\mathbb{N}$ and: 
\begin{align*}
%     u(t,x) &= \sum_{k=0}^{\infty} \hat{u}_k(t) \exp(-i k x) \\
    \hat{u}_k(t) &:= \int_0^{2\pi} u(t,x) \exp(-i k x) dx
\end{align*}

On the other hand, assume we have a discretized grid in $[0, 2 \pi]$ and a resolution $f$. Let $f_c = \floor{\frac{f-1}{2}}$ and $T = f^{-1}$. We are allowed to observe the function $u$ at points $\{x_n = n 2\pi T | n \in 0, .., f\}$ for every $t$. Let $\bar{u}$ be the discrete fourier transform:
$$
\bar{u}_{k} (t) := \sum_{n=0}^f u(t, x_n) \exp( -i 2 \pi n \frac{k}{f}  ) \quad |k| \leq f_c
$$

Applying the Poisson Summation formula, we have: 
\begin{align*}
    \bar{u}_k (t) = f \sumk \hat{u}_{k'}(t)
\end{align*}

Then, we can write the system of ODEs: 
\begin{align}
\label{lemma:ubar_t}
    \partial_t \bar{u}_k (t)  = \sumk
    f C_{k'} \ \hat{u}_{k'}\left(t\right)
\end{align}

Following the Mori-Zwanwig formalism, we would like to define observed variables $\alpha_k(t)$ and unobserved variables $\beta_k(t)$ that follow a dynamical system:
\begin{align*}
    % \label{lemma:mzdef} \nonumber
    \partial_t \alpha(t) = A_{11}(t) \alpha(t) + A_{12}(t) \beta(t) \\ 
    \partial_t \beta(t) = A_{21}(t) \alpha(t) + A_{22}(t) \beta(t)
\end{align*}

Given the discretized nature of our problem, the only observed quantities are $\hat{u}_k(t)$, so we naturally define $\alpha_k(t):=\bar{u}_k(t)$. On the other hand, the full system is determined by $\hat{u}_k(t)$, so we need to be able to recover $\hat{u}_k(t)$ from $\alpha_k(t)$ and $\beta_k(t)$. Thus, we define the unobserved variables as: $\beta_k(t) :=\hat{u}_k(t) - \gamma(t)\bar{u}_k(t)$ for some $\gamma(t) \in \mathbb{C}$. We are interested in describing the system with observed variables as much as possible, so we choose $\gamma(t)$ to minimize $||\beta_k(t)||$, yielding:
$$
\gamma(t) = \frac{\langle \hat{u}_k(t), \bar{u}_k(t) \rangle}{||\bar{u}_k(t)||^2} $$

Where $\langle \cdot, \cdot \rangle$ and $|| \cdot ||$ are taken in the $\ell^2(\mathbb{Z})$ space of square-summable complex sequences indexed by $k$. 
Given our definitions for $\alpha_k(t)$ and $\beta_k(t)$, using $\hat{u}_k (t)= \gamma(t) \alpha_k(t) + \beta_k(t)$ and applying \ref{lemma:uhat_t} and \ref{lemma:ubar_t}, we can derive: 

\begin{align*}
    \partial_t \alpha_k(t) & = f \sumk C_{k'} \hat{u}_{k'}(t) = f \sumk C_{k'} \left[ \gamma(t) \alpha_k(t) +  \beta_k(t) \right] \\
\end{align*}

And: 

\begin{align*}
    \partial_t \beta_k(t) & = C_k \hat{u}_k(t) - \gamma'(t) \bar{u}_k(t) - \gamma(t) f \sumk  C_{k'} \hat{u}_{k'}(t) \\
    & = \sumk \left[ C_{k'}\gamma(t)\delta_{kk'} - \gamma'(t)\delta_{kk'} - C_{k'} \gamma^2(t) f  \right] \alpha_{k'}(t) + \sumk \left[C_{k'}\delta_{kk'} - f \gamma(t) C_{k'}\right]\beta_{k'}(t)
\end{align*}

Now recall that in our setting, $\bar{u}_k=0$ for $|k|>f_c$, so the equations are simplified to: 
\begin{align*}
    \partial_t \alpha_k(t) & = f C_k \gamma(t) \alpha_k(t) + f \sumk C_{k'}\beta_{k'} (t) \\
    \partial_t \beta_k(t) & =
        \mathbf{1}(|k|\leq f_c) \left[C_k \gamma(t) (1 - f\gamma(t)) - \gamma'(t) \right]\alpha_k(t) + \sumk \left[C_{k'}\delta_{kk'}- f \gamma(t) C_{k'}\right]\beta_{k'}(t)
\end{align*}

This can be transformed into a generalized Langevin equation by integrating the ODE for $\beta$ and plugging the solution in the ODE for $\alpha$, resulting in a Markov term, a memory term, and a noise term. The importance of the memory term will be related to the product of the cross terms $fC_{k}$ and $\left[C_k \gamma(t) (1 - f\gamma(t)) - \gamma'(t) \right]$. In particular, when the maximum frequency of $u(t,x)$ is below $f_c$, then $\bar{u}_k(t) = f\hat{u}_k(t)$, so $\gamma(t) = \frac{1}{f}$ and the second term  $\left[C_k \gamma(t) (1 - f\gamma(t)) - \gamma'(t) \right]$ will be null. Therefore, there would be no memory effect. Conversely, if $u$ has frequencies beyond the critic one, then $\bar{u}$ and $\hat{u}$ will not be proportional, the memory term might be important.
